Effective Unsupervised Domain Adaptation with Adversarially Trained Language Models

Recent work has shown the importance of adaptation of broad-coverage contextualised embedding models on the domain of the target task of interest. Current self-supervised adaptation methods are simplistic, as the training signal comes from a small percentage of \emph{randomly} masked-out tokens. In this paper, we show that careful masking strategies can bridge the knowledge gap of masked language models (MLMs) about the domains more effectively by allocating self-supervision where it is needed. Furthermore, we propose an effective training strategy by adversarially masking out those tokens which are harder to reconstruct by the underlying MLM. The adversarial objective leads to a challenging combinatorial optimisation problem over \emph{subsets} of tokens, which we tackle efficiently through relaxation to a variational lowerbound and dynamic programming. On six unsupervised domain adaptation tasks involving named entity recognition, our method strongly outperforms the random masking strategy and achieves up to +1.64 F1 score improvements.

==> alg-DP.tex <==

\begin{algorithm}[tb]
\small
\textbf{Function:} calcPartitionTable \\
\textbf{Input}: Training datapoint $\vx$, teacher $\pi_\phi$, $K$\\
% \textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: DP table $\mathcal{Z}$
\begin{algorithmic}[1]
\FOR {$j=1$ \textbf{to} $N$} 
    \STATE $\mathcal{Z}[j,0] = 1 $
\ENDFOR
\FOR {$k=1$ \textbf{to} $K$} 
    \STATE $\mathcal{Z}[N-k+1,k] = \prod_{i=N-k+1}^N\pi_\phi(i|\vx)$
\ENDFOR
\FOR {$k=1$ \textbf{to} $K$}
    \FOR {$j=N-K$ \textbf{to} $1$}
        \STATE $\mathcal{Z}[j,k] = \mathcal{Z}[j+1,k] + \pi_\phi(j|\vx)\mathcal{Z}[j+1,k-1]$
    \ENDFOR
\ENDFOR
\end{algorithmic}
\caption{\small Dynamic Programming Table Calculation \reza{plz update to make the notation neat}}
\label{alg:dp-table}
\end{algorithm}

==> tab-da-result.tex <==
\begin{table*}[]
\begin{center}
\scalebox{0.83}{
\begin{tabular}{crrrr|rrrr|r|rrrr}
\toprule
 & \multicolumn{4}{c|}{\textbf{Unsup. DA}} & \multicolumn{4}{c|}{\textbf{Unsup. DA + in-domain}} & \multicolumn{1}{c|}{\textbf{Task}}  & \multicolumn{4}{c}{\textbf{Sup. DA + in-domain}}\\
\multicolumn{1}{c}{Task} & 
\multicolumn{1}{c}{rand} & \multicolumn{1}{c}{pos} & \multicolumn{1}{c}{ent} & \multicolumn{1}{c|}{adv} & \multicolumn{1}{c}{rand} & \multicolumn{1}{c}{pos} & \multicolumn{1}{c}{ent} & \multicolumn{1}{c|}{adv} & 
\multicolumn{1}{c|}{\textbf{Tuning}}&
\multicolumn{1}{c}{rand} & \multicolumn{1}{c}{pos} & \multicolumn{1}{c}{ent} & \multicolumn{1}{c}{adv} \\
\midrule
wnut2016 &	 47.11 & 46.79 & 46.95 & 47.03 & 46.93 & 47.69 & 47.84 & 48.01 & 63.16 & 58.57 & 57.93 & 58.4 & 58.98 \\
fin  & 21.55 & 22.53 & 22.73 & 23.38 & 21.7 & 26.7 & & & 83.22 & 84.48 & 84.69 & 84.31 & 84.73 \\
jnlpba  & 27.44 & 28.06 & 28.22 & 30.06 & 29.92 & 30.56 & 30.47 & 30.31 & 77.65 & 78.45 & 78.45 & 78.45 & 78.46\\
bc2gm  & 28.31 & 28.5 & 31.81 & 29.01 & 31.13 & 31.85 & 31.83 & 32.38 & 75.71 & 78.98 & 79.97 & 80.09 & 79.94 \\
bionlp09  & 26.37 & 27.53 & 29.21 & 29.24 & 31.38 & 31.03 & 34.33 & 35.05 & 82.73 & 84.25 & 85.33 & 85.29 & 84.9 \\
bionlp11epi & & & & & & & & & 75.23 & 79.14 & 78.61 & 78.47 & 79.30 
\bottomrule
\end{tabular}}
\caption{F1 score of NER span prediction tasks in several domain adaptation scenarios, (i)~\textbf{Unsup. DA}: unsupervised domain adaptation without using additional data; (ii)~\textbf{Unsup. DA + in-domain}: unsupervised domain adaptation with additional in-domain data from target task; (iii)~\textbf{Task tuning}: fine-tuning BERT on target domain which is the upper-bound of unsupervised domain adaptation; and (iv)~\textbf{Sup. DA + in-domain}: domain adaptation with in-domain data following by target task adaptation. We also vary the masking strategies in domain-adaptation phase.}
\label{tab:uda}
\end{center}
\end{table*}

% \begin{table*}[]
% \begin{center}
% \scalebox{1}{
% \begin{tabular}{lrrrrrr}
% \toprule
%  & Random  & POS & entropy & adv  \\
% \midrule
% wnut2016 &  \\
% fin &   \\
% jnlpba &   \\
% bc2gm &   \\
% bionlp09 &  
% \bottomrule
% \end{tabular}}
% \caption{Supervised domain adaptation scenario}
% \label{tab:supevised domain adaptation}
% \end{center}
% \end{table*}


% % \begin{table*}[]
% % \begin{center}
% % \scalebox{1}{
% % \begin{tabular}{lrrrrrrrr}
% % \toprule
% % &  Mask Strategy & Precision & Recall & F1 \\
% % \midrule
% % Domain adaptation & random & 48.06 & 66.41 & 55.77 \\
% %             & entropy & 50.41 & 67.95 & 57.89 \\
% %             & adversarial & 52.05 & 67.62 & \textbf{\textit{58.83}} \\
% % \hline            
% % %Adapt-CoNLL & target & rand & 66.02 & 61.76 & 63.82 \\
% % %            & & entropy & 64.05 & 58.79 & 61.31  \\
% % %            & & adv & 65.50 & 60.18 & 62.72  \\
% % Task adaptation & N/A & 64.95 & 61.47 & 63.16  \\
% % \midrule
% % Domain + task adaptation  & rand & 66.49 & 60.84 & 63.54  \\
% %             & entropy & 65.18 & 62.25 & 63.68  \\
% %             & adversarial & 65.56 & 63.57 & \textbf{64.55}  \\
% % \bottomrule
% % \end{tabular}}
% % \caption{Named entity segmentation on the WNUT test set. We compare our approach against finetuned BERT-base without domain adaption and other masking strategies in 3 adaptation scenarios: (i) adapt BERT-base model on CoNLL+WNUT data and tune on CoNLL training data, (ii) adapt BERT-base model on WNUT+500K tweets data and tune on WNUT training data}
% % \label{tab:wnut-result}
% % \end{center}
% % \end{table*}


==> tab-datasets.tex <==
\setlength\tabcolsep{1.5pt} % default value: 6pt
\begin{table}[t]
\small
\begin{center}
\scalebox{1}{
\begin{tabular}{l||lc|lc}
\toprule
&\multicolumn{1}{c}{\textbf{NER}} & \multicolumn{1}{c}{\textbf{tokens/sent.}} & \multicolumn{1}{|c}{\textbf{Unlab.}} &\multicolumn{1}{c}{\textbf{tokens}}\\
\multicolumn{1}{c||}{\textbf{Domain}} & \multicolumn{1}{c}{\textbf{Dataset}} & %\multicolumn{1}{c}{\textbf{Train}} & 
%\multicolumn{1}{c}{\textbf{Dev.}} & 
\multicolumn{1}{c}{\textbf{Test}} & \multicolumn{1}{|c}{\textbf{Corpus}} & \multicolumn{1}{c}{\textbf{/sent.}} \\
\midrule
\textsc{News} & CoNLL2003 &  46.4k/3.5k  \\
\textsc{Tweet} & WNUT2016 &  61.9k/3.8k & Sentiment140 & 20M/1.4M\\
\textsc{Fin} & FIN        &  13.3k/303 & {\scriptsize SECSEC Filing 2019} & 155M/5.5M \\
\textsc{BioMed}               & JNLPBA  &  101.0k/3.9k  & PubMed & 4.3B/181M\\
\textsc{BioMed}  & BC2GM  &  143.5k/5.0k  & PubMed & 4.3B/181M \\
\textsc{BioMed}  & BioNLP09 &  74.6k/2.5k & PubMed & 4.3B/181M\\   
\textsc{BioMed}  & BioNLP11EPI &  116.1k/4.1k & PubMed & 4.3B/181M\\
\bottomrule                 
\end{tabular}
}
\caption{Data statistics of named entity span prediction tasks and unlabled additional pretraining corpus.}
\label{tab:dataset}
\end{center}
\end{table}



% \begin{table}[]
% \begin{center}
% \scalebox{1}{
% \begin{tabular}{lcrr}
% \toprule
% Dataset & Domain  & \#tokens & \#sent  \\
% \midrule
% Sentiment140 & tweet &  & 1.4M \\
% SEC filing 2019 & financial &  & 5.5M \\
% Pubmed & biomedical & &   \\
% \bottomrule
% \end{tabular}}
% \caption{Pretraining corpus}
% \label{tab:mix-strategy}
% \end{center}
% \end{table}
